Flexible Marginal Models for Dependent Data

Models for dependent data are distinguished by their targets of inference. Marginal models are useful when interest lies in quantifying associations averaged across a population of clusters. When the functional form of a covariate-outcome association is unknown, flexible regression methods are needed to allow for potentially non-linear relationships. We propose a novel marginal additive model (MAM) for modelling cluster-correlated data with non-linear population-averaged associations. The proposed MAM is a unified framework for estimation and uncertainty quantification of a marginal mean model, combined with inference for between-cluster variability and cluster-specific prediction. We propose a fitting algorithm that enables efficient computation of standard errors and corrects for estimation of penalty terms. We demonstrate the proposed methods in simulations and in application to (i) a longitudinal study of beaver foraging behaviour, and (ii) a spatial analysis of Loaloa infection in West Africa. R code for implementing the proposed methodology is available at https://github.com/awstringer1/mam.

==> sections/042-computations.tex <==
%!TEX root = ../MMM_draft.tex

\section{Computation}\label{s:computation}

Our recommended computational strategy for fitting MAMs is given in Algorithm ... We adopt the mixed model framework \citep[\S6.6]{wood2017generalized} for fitting GAMMs. We describe the details in \S\ref{ss:conditionalmodelgamm}, with emphasis on how this approach naturally provides the necessary quantities for making point and interval estimates for $\smoothfunMest$ using Theorem \ref{thm:convergence}. Naive calculation of standard errors for $\smoothfunMest$ requires inversion of a dense $n\times n$ matrix, having computational complexity of $O(n^{3})$ and memory usage of $O(n^{2})$, and hence becoming computationally prohibitive as $n=\sum_{i=1}^{\numclusters}\numunits_{i}$ increases. In \S\ref{ss:standarderrors} we exploit the structure of $\smoothfunMest$ to give an algorithm for computing standard errors having computational complexity of order ...


\subsection{Fitting the Conditional Model}\label{ss:conditionalmodelgamm}



\subsection{Standard Errors}\label{ss:standarderrors}

\subsection{Transformation of Random Effects}\label{ss:transformationrandomeffects}

(talk about Gaussian transformation)



==> sections/05-01-resp.tex <==
%!TEX root = ../MMM_draft.tex

\subsection{Longitudinal Study of Respiratory Health}
\label{ss:app1}
\glen{I think this could end up in the supplementary material. Unfortunately this is an RCT, so age isn't a \textit{confounder}, rather a precision variable. So we wouldn't expect the treatment effect to change much based on different specifications of the age association.}



\citet{geepack} consider the following mean model for a longitudinal trial of a treatment for respiratory illness:
\begin{equation}\label{eqn:respiratorymarginalmean}
\logit\left\{\EE(\responsei_{ij})\right\} = \covx_{i}\tpose\margbeta + \smoothfunM(\texttt{age}_{i}).
\end{equation}
Here $\responsei_{ij}$ is a binary indicator of whether the respiratory state of patient $i=1,\ldots,56$ at visit $j=1,\ldots,4$ is ``good''; $\covx_{i} = (x_{1i},\ldots,x_{4i})$ are covariates including which of two centres the patient visited, their sex, whether they received the treatment or a placebo, and a binary indicator of their baseline respiratory status, and $\margbeta = (\margbetai_{0},\ldots,\margbetai_{4})$; and $\texttt{age}_{ij}$ is the age of patient $i$ in years. All the covariates are constant within patient, across visits. 

The estimand of interest is the population-averaged association between treatment with the log-odds of having ``good'' respiratory status, $\margbetai_{3}$. Although the other covariates are prognostic in nature,  \citet{hastieprognostic} argued that improper modelling of prognostic factors can negatively affect estimation of treatment effects. And as \citet{geepack} pointed out, respiratory status appears to vary with age non-linearly; see Figure \ref{fig:resp-plots} (top panel).


\citet{geepack}  modelled  $\smoothfunM(\cdot)$ as a quadratic. To avoid assuming a specific functional form, we fit a MAM with the mean structure given by (\ref{eqn:respiratorymarginalmean}), where $\smoothfunM(\cdot)$ is represented by a thin plate regression spline basis \citep{thinplatesplines} of rank 10. For comparison, we also fit two MMMs, which assume quadratic and cubic structures for $\smoothfunM(\cdot)$, respectively. All models incorporated random intercepts.


Figure \ref{fig:resp-plots} (bottom row) shows estimates and 95\%  confidence intervals for $\smoothfunM(\cdot)$ under the three models. The MAM estimates were substantially more attenuated and its intervals were narrower than those those of the MMM polynomial models.   Despite the differences in estimated age associations, coefficient estimates for other prognostic factors were similar across models (see Table \ref{tab:resp-table}). Ultimately, the MAM estimate of the treatment effect differed modestly from the quadratic MMM estimate (by more than 50\% the corresponding standard error). One could of course fit several polynomial MMMs and select a best model via hypothesis testing, but this would require adjustment for post-selection inference. The MAM, by contrast, approach estimates $\smoothfunM(\cdot)$ automatically.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.35\linewidth]{../Code/Plots/respiratory_loess} \\
	\includegraphics[width=0.99\linewidth]{../Code/Plots/respiratory_panels}
	\caption{Top panel: prevalence of good respiratory status per subject by age \S\ref{ss:app1}. Bottom row: estimates and pointwise standard error bands for $\smoothfunM(\texttt{age})$. The MAM estimates the function via a flexible basis expansion and penalized regression; MMMs force the function to have a quadratic ($d=2$) or cubic ($d=3$) shape.}
	\label{fig:resp-plots}
\end{figure}

\begin{table}[htbp!]
	\centering
\caption{Coefficient estimates and standard errors for the respiratory analysis of \S\ref{ss:app1}. $d$ refers to the degree of the polynomial structure assumed for the age association in the MMMs.}
\label{tab:resp-table}
	\begin{tabular}{l r@{\extracolsep{5pt}}r r@{\extracolsep{5pt}}r r@{\extracolsep{5pt}}r}
		\toprule
Covariate & \multicolumn{1}{c}{MAM} & \multicolumn{1}{c}{MMM ($d=2$)} & \multicolumn{1}{c}{MMM ($d=3$)} \\
		\midrule
		Baseline & 1.510 (0.279) & 1.690   (0.288) &1.6871   (0.2879)      \\
		Centre & 0.517 (0.228) & 0.526    (0.236) & 0.5520   (0.2380)      \\
		Sex (Male) & -0.479 (0.351) & -0.517    (0.354)  & -0.5682   (0.3619)     \\
		Treat. (Plac.) & -1.357 (0.270) & -1.511    (0.276)  & -1.4903   (0.2766)     \\
				\hline
	\end{tabular}


\end{table}



